Density of weak solutions of the fractional Navier-Stokes equations in the smooth divergence-free vector fields

In this paper, we consider the fractional Navier-Stokes equations. We extend a previous non-uniqueness result due to Cheskidov and Luo, found in [5], from Navier-Stokes to the fractional case, and from $L^1$-in-time, $W^{1,q}$-in-space solutions for every $q > 1$ to $L^s$-in-time, $W^{1,q}$-in-space solutions for appropriate ranges of $s,q$.

==> newtxstuff.tex <==
\makeatletter
\newif\iftx@coch
\newif\iftx@ch
        \RequirePackage[T1]{fontenc}
        \ExplSyntaxOn
        \expandafter\str_if_eq:nnTF\expandafter{\mw@ptmx}{empty}{
        \def\mw@do#1{\def#1{\csname x\expandafter\@gobble\string#1\endcsname[b]}}
        \mw@do\ag
        \mw@do\bg
        \mw@do\gg
        \mw@do\dg
        \mw@do\eg
        \mw@do\zg
        \mw@do\hg
        \mw@do\qg
        \mw@do\ig
        \mw@do\kg
        \mw@do\lg
        \mw@do\mg
        \def\ng{\xng[b]}
        \mw@do\jg
        \mw@do\og
        \mw@do\pg
        \mw@do\rg
        \mw@do\sg
        \mw@do\tg
        \mw@do\ug
        \mw@do\fg
        \mw@do\xg
        \mw@do\yg
        \mw@do\wg
        }{}
        \renewcommand{\rmdefault}{ntxrx}
        \newif\iftx@libertine\tx@libertinefalse
        \newif\iftx@minion\tx@minionfalse
        \newif\iftx@ams\tx@amsfalse
        \newif\iftx@slantedG\tx@slantedGfalse
        \newif\iftx@cmint\tx@cmintfalse
        \newif\iftx@braces\tx@bracesfalse
        \newif\iftx@varbb\tx@varbbfalse
        \newif\iftx@vvarbb\tx@vvarbbfalse
        \newif\iftx@symbolsC\tx@symbolsCtrue
        \newif\iftx@gm\tx@gmfalse
        \newif\iftx@altnu\tx@altnufalse
        \newif\iftx@largelibfigs\tx@largelibfigsfalse
        \newif\iftx@libaltvw\tx@libaltvwfalse
        %\RequirePackage{newtxmath}    Problems, problems everywhere…
        \RequirePackage{fontaxes}
%        \DeclareSymbolFont{operators}{\encodingdefault}{\rmdefault}{m}{n}
%        \SetSymbolFont{operators}{bold}{\encodingdefault}{\rmdefault}{b}{n}
\DeclareSymbolFont{operators}   {OT1}{ztmcm}{m}{n}
        \def\operator@font{\mathgroup\symoperators}
        \DeclareMathAlphabet{\mathsf}{\encodingdefault}{\sfdefault}{m}{n}
        \DeclareMathAlphabet{\mathit}{\encodingdefault}{\rmdefault}{m}{it}
        \DeclareMathAlphabet{\mathtt}{\encodingdefault}{\ttdefault}{m}{n}
        \DeclareSymbolFontAlphabet{\mathrm}{operators}
        \DeclareMathAlphabet{\mathbf}{\encodingdefault}{\rmdefault}{b}{n}
        \SetMathAlphabet{\mathit}{bold}{\encodingdefault}{\rmdefault}{b}{it}
        \SetMathAlphabet{\mathsf}{bold}{\encodingdefault}{\sfdefault}{b}{n}
        \SetMathAlphabet{\mathtt}{bold}{\encodingdefault}{\ttdefault}{b}{n}
        %\DeclareSymbolFont{txletters}{OML}{ntxmi}{m}{it}
        %\SetSymbolFont{txletters}{bold}{OML}{ntxmi}{b}{it}
        %\DeclareFontSubstitution{OML}{ntxmi}{m}{it}
        %Commenting these out allows for choice of \mathcal alphabet…
        \def\defaultscriptratio{.73} % default is .7
        \def\defaultscriptscriptratio{.55} % default is .5
        \DeclareMathSizes{5}    {5.5}    {5.5}    {5.5}
        \DeclareMathSizes{6}    {6.5}    {5.5}    {5.5}
        \DeclareMathSizes{7}    {7.3}    {5.5}    {5.5}
        \DeclareMathSizes{8}    {8}    {6.2}    {5.5}
        \DeclareMathSizes{9}    {9}    {7.3}    {5.5}
        \DeclareMathSizes{10}   {10}   {7.3}  {5.5} 
        \DeclareMathSizes{10.95}{10.95}{8}    {6.1}
        \DeclareMathSizes{11}   {10.95}{8}    {6.1}
        \DeclareMathSizes{12}   {12}   {8.8}    {6.6}
        \DeclareMathSizes{14.4} {14.4} {10.5}   {7.9}
        \DeclareMathSizes{17.28}{17.28}{12.5}   {9.4}
        \DeclareMathSizes{20.74}{20.74}{16.1} {11.4}
        \DeclareMathSizes{24.88}{24.88}{18.2}{13.7}
        \DeclareMathSymbol{\omicron}{\mathord}{operators}{`\o}
